Probabilistic Neural Data Fusion for Learning from an Arbitrary Number of Multi-fidelity Data Sets

In many applications in engineering and sciences analysts have simultaneous access to multiple data sources. In such cases, the overall cost of acquiring information can be reduced via data fusion or multi-fidelity (MF) modeling where one leverages inexpensive low-fidelity (LF) sources to reduce the reliance on expensive high-fidelity (HF) data. In this paper, we employ neural networks (NNs) for data fusion in scenarios where data is very scarce and obtained from an arbitrary number of sources with varying levels of fidelity and cost. We introduce a unique NN architecture that converts MF modeling into a nonlinear manifold learning problem. Our NN architecture inversely learns non-trivial (e.g., non-additive and non-hierarchical) biases of the LF sources in an interpretable and visualizable manifold where each data source is encoded via a low-dimensional distribution. This probabilistic manifold quantifies model form uncertainties such that LF sources with small bias are encoded close to the HF source. Additionally, we endow the output of our NN with a parametric distribution not only to quantify aleatoric uncertainties, but also to reformulate the network's loss function based on strictly proper scoring rules which improve robustness and accuracy on unseen HF data. Through a set of analytic and engineering examples, we demonstrate that our approach provides a high predictive power while quantifying various sources uncertainties.

==> 12_Intro.tex <==
\section{Introduction} \label{sec:intro}
This is the intro and here we want to reference to Figure \ref{fig:multiscale}.
As you see here, we can also refer to a section, e.g., Sec. \ref{sec:research}) and cite papers very easily \cite{RN1516, RN1521, RN1522, RN1523}.
To start a new paragraph, we need to have an empty line or use $//$!
%=================================================================================
\begin{figure*}[!b] 
	\centering
	\includegraphics[page=1, width = 0.8\textwidth]{Figures/Multiscale.pdf}
	\vspace{-0.3cm}
	\caption{\textbf{Preliminary results:} The macro-structure has $451,932$ integration points (IPs). Each IP corresponds to a unique microstructure whose deformations are modeled via a pre-trained LEGO.}
	\label{fig:multiscale}
\end{figure*}
%=================================================================================




%=================================================================================
\begin{wrapfigure}{r}{0.55\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{Figures/vision.pdf}
    \vspace{-0.7cm}
    \caption{\textbf{Envisioned CF:} The user $(1)$ selects the PDE types that govern the application, and $(2)$ determines the domain, ICs, BCs, and other application-dependent parameters. Next, our algorithm chooses the LEGOs that approximate the PDE solutions in a genome. Finally, BRL is used to couple genome-wise predictions to approximate the solution in the domain while ensuring solution consistency.}
    \label{fig:flowchart}
\end{wrapfigure}
%=================================================================================
\noindent \textcolor{navy}{\textbf{Removing indent and making a sentence bold with a specific color.}} You can also make \textit{wrapped} figures such as \ref{fig:flowchart}. Some random text: Over the past few years, these attractive properties of DNNs have sparked on many fundamental and applied works. In solid mechanics and materials science, DNNs have been used to learn the path-dependent and irreversible deformation of nonlinear materials \cite{RN1211, RN1024, RN907, RN908}, design optimum tool path in additive manufacturing \cite{RN785}, estimate unknown material properties \cite{RN1432}, emulate material fracture \cite{RN1419}, or coarse-grain material models \cite{RN918, RN919, RN920, RN1005, RN1006, RN1007, RN1008, RN1009, RN1010, RN1013, RN1036, RN1037, RN1038, RN1064, RN1116, RN1130, RN1231, RN1232, RN1233, RN1234}. 
In fluid dynamics and thermal analysis, DNNs are increasingly used for forward and inverse flow field approximation in channels of various shapes and sizes (including human veins) \cite{RN833, RN835, RN1066, RN1068, RN1069, RN1110, RN1112, RN1162, RN1169, RN1173, RN1204}, optimal flow control and UQ \cite{RN1143, RN1100, RN836}, or climate and cloud modeling \cite{RN1467, RN1468, RN1472, RN1358, RN1311, RN1312, RN1313, RN1314, RN1315, RN1316, RN1317}. 
While these and other recent works have substantially advanced the field, \ul{two primary limitations still exist}: 

\section{Technical Background} \label{sec:back}
A new section. {\Large See how I label sections, figures, tables, ...: They start with fig:, sec:, ... so we can find them easily!}.

 To demonstrate how equations are written, consider the boundary value problem (BVP):
\vspace{-0.2cm}
%=================================================================================
\begin{align}
    \nabla^2u(\pmb{x}) &= 0,  \qquad\; \pmb{x}\in\Omega \hspace{2cm} \\
    u(\pmb{x}) &= g(\pmb{x}), \quad \pmb{x}\in\partial\Omega
    \vspace{-0.2cm}
    \label{eqn:ex_laplace}
\end{align}
%=================================================================================
where $\pmb{x}=[x, y, z]$, $\nabla^2$ is the Laplacian operator,
%($\partial^2/\partial x^2 + \partial^2/\partial y^2$)
$\Omega$ denotes the domain with boundary $\partial\Omega$, and $g(\pmb{x})$ defines the BC. When training a DNN that approximates $u(\pmb{x})$, the loss function can be designed as:
\vspace{-0.1cm}
%=================================================================================
    \begin{gather}
        L(\hp) = L_1(\hp) + \alpha L_2(\hp) + \beta L_3(\hp),\\
        L_1(\hp) = \frac{1}{N_1}\sum^{N_1}_{i=1} 
                   \left ( u(\pmb{x}_i) - \nn(\pmb{x}_i|\hp) \right )^2,  \nonumber \hspace{0.8cm}
        L_2(\hp) = \frac{1}{N_2}\sum^{N_2}_{j=1}
                      \left ( \nabla^2\nn(\pmb{x}_i|\hp) \right )^2, \hspace{0.8cm}
        L_3(\hp) = |\hp|^2 
    \vspace{-0.1cm}
    \label{eqn:ex_pinn_loss}
    \end{gather}
%=================================================================================
where $\hp$ are the network parameters, $\nn$ denotes the DNN, $L_1(\hp)$ is the error in reproducing the training data obtained from traditional solvers, $L_2(\hp)$ is the residual which enforces $\nn$ to satisfy the Laplace equation on some randomly selected points (aka collocation points) in $\Omega$, $L_3(\hp)$ denotes Tikhonov regularization that prevents overfitting, and $\alpha$ and $\beta$ are constants that control the contributions of, respectively, $L_2(\hp)$ and $L_3(\hp)$ to $L(\hp)$. $L_2(\hp)$ in Equation \ref{eqn:ex_pinn_loss} involves partial derivatives which can be analytically calculated via AD.


\section{Proposed Research} \label{sec:research}
Our framework has a ....
In our preliminary studies we have fixed the genome shape to a small square and adopted an iterative approach for coupling genome-wise predictions. Our choices on genome shape and size simplified the data collection and training process by limiting the number of DNN's inputs and trainable parameters. The iterative approach is an advanced version of Schwarz's method \cite{RN1531} which guarantees convergence to the ground truth \cite{RN1516, RN1521, RN1523} as long as the genome-wise solutions are estimated sufficiently accurately. We implemented this iterative approach via \textbf{basic and auxiliary genomes}: the basic ones span the domain with as little overlap as possible while the auxiliary ones accelerate information propagation across the basic genomes, see Figure \ref{fig:iteration_laplace}. The placement of these genomes was controlled manually and will be automated via BRL in this project. Using this sub-optimal iterative approach, we have been able to solve the Laplace equation in a domain that is not only more than $1200$ times larger than the training domain (i.e., the genome), but also has a BC that is not seen during training. We have also been able to scale up our approximations in solving the NS equations by $12$ times while preserving complex flow features that are never seen during training.

%=================================================================================
\begin{figure}[!t]
    \centering
    \subfloat[Domain consists of 4 non-overlapping basic genomes which are covered via 5 auxiliary genomes. \label{fig:iteration_laplace}]
    {\includegraphics[width=0.8\textwidth]{./Figures/Iterations_laplace.pdf}}\\[-0.5mm]
    \subfloat[The logo of mosaic flow whose area is $1200 \times$ larger than the genome. \label{fig:1200laplace}]
    {\input{./Figures/MF_logo/Logo_SC_Figure.tex}}\\[-3mm]
    \caption{\textbf{Self-adaptive coupling of a LEGO:} The LEGO learns the Laplacian operator in $\Omega$ ~for arbitrary $g(x, y)$. The self-adaptive mechanism iteratively uses this LEGO to find the solution in a very large domain under unseen BCs. A hybrid coupling mechanism that leverages optimization and BRL will be developed in this project.}
    \label{fig:laplace}
\end{figure}
%=================================================================================

In addition to providing transferability and scalability, \ul{our contributions are expected to increase the accuracy of DNNs in approximating PDE solutions}. Currently, DNNs provide at least $5$ orders of magnitude less accuracy compared to high-fidelity expensive numerical solvers which use the FE, FV, or FD methods. This massive gap in accuracy is due to a number of factors. For example, DNNs that emulate PDE solutions are generally trained via single precision computations because the search for optimal architecture and parameters would be otherwise too computationally prohibitive and memory intensive. 
Another related factor is the use of mini-batch stochastic gradient descent (SGD) in DNN training which fails to sufficiently reduce PDE residuals that rely on high-order partial derivatives. These errors are highly sensitive to gradients and thus require second-order optimization routines that employ the (approximate) Hessian matrix of the loss function. 
By limiting the emulation to the genome scale, the number of trainable parameters of our DNNs are much smaller than existing networks that aim to approximate PDE solutions (while smaller, our DNNs will possess a much higher parameter to domain size ratios and thus are expected to provide more learning capacity). Additionally, collecting data on genomic scales (see Sec. \ref{sec:deep_learning}) is much simpler and computationally less expensive compared to existing practices where the collected data set is application dependent. \ul{With smaller networks and more training data, we are able to use double precision computations and leverage second-order gradient-based optimization techniques to approach the same level of accuracy provided by traditional numerical solvers}. 

Our LEGOs are operator surrogates that learn a PDE parametrically, i.e., they are agnostic to the ICs and BCs applied to the genome. We build these LEGOs in \hyperref[sec:task1]{\textbf{Research Thrust 1}} and endow them with novel architectures that break the curse of dimensionality. In \hyperref[sec:task2]{\textbf{Research Thrust 2}}, we develop the methods and algorithms for coupling the LEGOs to model multi-physics systems or spatiotemporally extrapolate their predictions. To achieve real-time performance and massive scalability on heterogeneous machines, we co-design our software with hardware accelerators in \hyperref[sec:task3]{\textbf{Research Thrust 3}}.

Recently, data-driven operator emulation via DNNs has drawn significant attention because operator learning provides much more generalization power than function learning. However, existing works \cite{RN1257, RN1509, RN1144} train single-physics surrogates with very limited transferability and no scalability. To address these limitations, \textbf{we develop a self-adaptive coupling mechanism based on BRL that $(1)$ spatiotemporally scales the predictions of a LEGO, and $(2)$ can couple multiple LEGOs that emulate different physics}. 
This decomposition-learning-coupling approach is supported by \textbf{two hypotheses} which will be tested:

\noindent\textbf{H1:} Within a genome, a LEGO can accurately learn complex, nonlinear transformations that map functionals from one space to functionals in another space.

\vspace{-2mm}
\noindent\textbf{H2:} Coupling LEGO-based predictions in multiple connected genomes rapidly transfers information; enabling spatiotemporal extrapolation and multi-physics modeling. 

The \textbf{rationale} behind \textbf{H1} is the universal approximation theorem of DNNs \cite{RN1421}. While hypotheses with similar arguments are recently posed \cite{RN1257, RN1509, RN1144}, applications have been limited to simple problems. We bridge this gap via two innovations:
$(1)$ our LEGOs' architecture and multi-stage training process that leverages mixed-precision computing, wealth of domain-agnostic data, and memory-efficient optimization routines, and 
$(2)$ our self-adaptive coupling mechanism in \textbf{H2} whose \textbf{rationale} is based on curriculum learning \cite{RN1157} which was originally developed to accelerate animal training \cite{RN1158, RN1156} by planning a learning process to begin by learning simple concepts that collectively constitute complex concepts. 
Correspondingly, our coupling mechanism uses reward functions to complete a difficult task (large-scale, multi-physics emulation in our case) by systematically decomposing it to simpler but interconnected tasks (small-scale, single-physics, coupled emulation in our case). This mechanism is automated by BRL and its associated computations are distinctly suited to distributed heterogeneous machines and are leveraged in \hyperref[sec:task3]{Research Task 3}.

In computational fluid dynamics, techniques known as multi-block methods (MBMs) \cite{RN1153, RN1155, RN1152, RN1154} have been developed that rely on domain decomposition mathematics. The primary goal of MBMs is to leverage parallel computing by decomposing a complex domain into sub-domains distributed across several computing nodes. The PDEs are then numerically solved (e.g., via FE or FD) in each sub-domain, and solution consistency across the sub-domain boundaries is ensured with periodic cross-domain inter-node communications. The major differences between our approach and MBMs are twofold. 
$(1)$ Computational costs and transferability: Since we use transferable pre-trained LEGOs, the costs of solution prediction in unseen domains are drastically lower compared to MBMs. Lower costs enable rigorous convergence studies and uncertainty analyses. 
$(2)$ Ease-of-use and versatility: MBMs heavily rely on optimized communication and load balancing. Moreover, their application in large-scale problems generally requires several convergence acceleration techniques such as multigrid, implicit residual smoothing, and local time stepping in addition to parallelization. Our approach does not rely on these advanced numerical techniques to ensure scalability. 

\subsection{Research Thrust 1: LEGOs Library (RB Leads)}\label{sec:task1}
The \textbf{goal} of this thrust is to validate hypothesis \textbf{H1} by building a rich library of LEGOs that approximate a wide range of PDE solutions on genomic domains. Thrust 1 is a key component of the framework because (a) the diversity of LEGOs increases ease-of-use and community-wide adoption, (b) the size and shape of the genomes directly affect the coupling mechanism and flexibility in domain decomposition, and (c) the predictive power of LEGOs determines the overall accuracy in large-scale applications. 

\subsubsection{Genomes}
\label{subsubsec:genomes}
We consider two broad classes of 2D/3D genomes: (a) rectangles/squares and cuboids/cubes with fixed sizes, and (b) parametrized shapes, see Figure \ref{fig:lego+nurb}(a) and (b). The first class of genomes will greatly benefit multi-scale simulations in solid mechanics (see Sec. \ref{sec:eval}) and will also streamline integrating Thrust 1 with Thrust 2 since it is simpler to approximate PDEs over them and conduct error analysis (see Sec. \ref{sec:error}). These genomes are also useful for spanning the interior or bounding box of large complex domains, see Figure \ref{fig:lego+nurb}(c). Our second class of genomes will be based on Bézier curves/surfaces \cite{RN1543, RN1544, RN1545, RN1546} and non-uniform rational basis spline (NURBS) that is widely used in isogeometric analysis which integrates FE with computer-aided design (CAD) tools \cite{RN1541, RN1542}. For instance, NURBS-based genomes can represent a large variety of shapes in 2D and 3D using control points and their corresponding weights \cite{RN1532, RN1533, RN1534}, see Figure \ref{fig:lego+nurb}(d). 

Similar to the parametrized shapes that will be quantified with a finite number of variables, we will also discretize ICs and BCs. The discretization is an important step that determines the number of DNN inputs and hence its overall size. To automate this process, and leverage the high correlation between the discretized functions (e.g., the control points can be shared between discretized BCs and NURBS), we will use supervised pre-training based on autoencoders, see Sec. \ref{sec:deep_learning}. 

%=================================================================================
\begin{figure}[!t]
    \centering
    \includegraphics[width=\textwidth]{Figures/LEGO+Nurbs.pdf}
    \vspace{-0.7cm}
    \caption{\textbf{LEGOs: (a)} With fixed geometry, a LEGO only needs ICs and BCs as inputs for solving the NS equations. \textbf{(b)} For a parametric geometry, additional inputs ($g$) characterizing the domain are needed. The high correlation between these inputs is leveraged during training, see Sec. \ref{sec:deep_learning}. The LEGOs in \textbf{(a)} and \textbf{(b)} solve the 2D NS equations where $p$ denotes flow-specific parameters. \textbf{(c)} Many sub-domains take on simple forms (e.g, rectangles) when decomposing a large domain. \textbf{(d)} NURBS characterize a generic 3D surface with a finite number of parameters. \textbf{(e)} Supervised pre-training reduces the dimensionality of complex shapes.} 
    \label{fig:lego+nurb}
\end{figure}
%=================================================================================

%=================================================================
\begin{wrapfigure}{r}{0.34\textwidth}
    \centering
    \vspace{-0.8cm}
    \includegraphics[width = 1\textwidth]{Figures/transient pde.pdf}
    \caption{\textbf{Transient PDE in a 2D space:} The flow's velocity magnitude in an elbow-shaped pipe is visualized on a regular grid (dots indicate where data is available). At $t=0$, a slow-speed flow ($u=1m/s$) enters the elbow through the inlet at $x=0$ and a high-speed flow ($v=3m/s$) is injected at the inlet at $y=0$. The flow mixes and exits the elbow via the top outlet.}
    \label{fig:transient}
\end{wrapfigure}
%=================================================================
With either genome class, the characteristic size of the genome, $L$, is an important parameter that presents some trade-offs. On the one hand the \textbf{offline} costs of obtaining training data and building LEGOs \emph{grow} as $L$ increases. On the other hand, the \textbf{online} costs of ensuring cross-genome solution consistency \emph{decrease} as $L$ increases. A similar behavior is observed in accuracy, i.e., with smaller genomes the errors of LEGOs and assembled predictions decrease and increase, respectively. Hence, the overall accuracy can be balanced as a function of $L$. 
The trend in the accuracy of LEGOs and assembled predictions is because with small $L$, a LEGO needs to learn the physics in a small region where possible solution variations are limited. If such a LEGO does not achieve sufficiently small residuals, the coupled predictions grow and dominate the overall error.
Our studies on error (see Sec. \ref{sec:error}) suggest that the optimum $L$ is the largest genome size that satisfies two conditions: 
(1) its discretization with a finite number of parameters does not result in information loss, and 
(2) LEGOs are small enough so they can be trained with descent batch sizes on GPUs.
In this project, we will address this computational bottleneck and minimize performance sensitivity to $L$ via supervised pre-training, ensembling, and multi-stage training on heterogeneous machines, see Sections \ref{sec:deep_learning}, \ref{sec:ensembling}, and \ref{sec:task3}. 
These discussions on $L$ are equally applicable to \textit{time intervals} in transient systems where time is considered as an additional dimension, see Figure \ref{fig:transient}. 

\subsubsection{Deep Learning}\label{sec:deep_learning}

\noindent \textcolor{navy}{\textbf{Data Collection.}} Given the high dimensionality and complexity of operator learning, we will generate a very large data set for training each LEGO (our preliminary studies indicate $> 10^4$ samples are needed, in addition to collocation points). \ul{This is a one-time offline cost that will be amortized by the repeated use of LEGOs in predictions across different applications}. We will use two methods for data generation which are motivated by PI Bostanabad's previous works in multiscale materials modeling \cite{RN704, RN1024}:

\vspace{-0.2cm}
\noindent \textbf{Method 1:} Sweeping available PDE solutions with a genome and recording the solution within the genome and on its edges/faces, see Figure \ref{fig:data_collection}(a). Genomes of various shapes/sizes will be used. In addition to online resources such as \cite{cgns-grids, stanford-grids} for flow fields, we have extensive data that can be used for this purpose \cite{cfdnet2020, wang2019multi, mostafazadeh2018roofline, mostafazadeh2017unsteady, RN6, RN545, RN704, RN1024, RN791, RN681, RN1384, RN1109}. This method is fast and easy-to-implement but it may not provide high data diversity. 

\vspace{-0.2cm}
\noindent \textbf{Method 2:} Generating the ICs, BCs, and other inputs (e.g., control points and weights of NURBS) via a random process (RF) as in Figure \ref{fig:data_collection}(b) and then using traditional solvers to gather solution data from the designed genome. This method can generate diverse training data by minimizing data correlations but is more expensive because we cannot a priori guarantee the generated BCs will yield feasible solutions. 

We will start the data collection by Method 1 to not only minimize the costs but also calculate the input ranges that are needed for Method 2 (e.g., max/min for pressure profile applied as BC for flow learning). Then, we will use Method 2 for data augmentation, i.e., if LEGOs have insufficient accuracy or if data is scarce in specific conditions (e.g., very high Reynolds numbers). 
With each method, we will use a wide range of genome shapes and sizes. For parametric genomes created via NURBS or Bézier curves we will ensure well-posedness by ensuring positional and tangential continuity conditions \cite{RN1535, RN1537, RN1538, RN1539, RN1540}.
Data augmentation costs will be quite manageable because the genomes are small and all simulations will be run in parallel. 

%=================================================================
\begin{figure}[!t]
    \centering
    \includegraphics[width = 1\textwidth]{Figures/data collection.pdf}
    \vspace{-0.7cm}
    \caption{\textbf{Data collection:} To learn the NS equations we gather data by \textbf{(a)} sweeping available flows with a genome (Method 1), and \textbf{(b)} generating the ICs/BCs with random processes and then solving the NS equations (Method 2). In \textbf{(b)}, five pressure profiles are generated via a random process to serve as the BCs in five simulations. Data from Method 1 determine $p_{min}$ and $p_{max}$.
    } \label{fig:data_collection}
\end{figure}
%=================================================================

\noindent \textcolor{navy}{\textbf{Architecture and Training.}}
It is widely accepted that the performance of a DNN greatly depends on its architecture and training procedure \cite{RN1070, RN248}. 
This sensitivity is even more pronounced for DNNs that approximate PDE solutions. For instance, we have observed \cite{RN1481} that in cavity simulations CNNs learn vortices better than FCFF networks while the latter more accurately represent near-wall conditions where velocity streamlines are tangent to the domain boundary. 
\ul{We are in a unique position to address this sensitivity issue through ensembling where we will use a wide range of network architectures and training procedures to build multiple LEGOs that learn the same PDE system}. While ensembling is a well-established and widely popular practice, it is rarely used in approximating PDE solutions via DNNs because the training costs are prohibitively high while the DNNs' transferability are very limited. However, our use of ensembling is justified because the LEGOs are \textit{trained once and intended to be used forever} within our framework. Correspondingly, we will use a wide range of architectures (CNNs, FCFFs, RNNs, ... with/without residual connections) and training procedures (e.g., with/without double-precision computation or Tikhonov regularization) to \ul{build multiple LEGOs that learn a specific PDE system}. Hence, the inferences from \textit{same physics} LEGOs will provide probabilistic predictions that are used in the BRL-based coupling mechanism. 

%Talk about enforcing BCs?

LEGOs' inputs are high-dimensional as they encode discretized BCs, ICs, and shapes, see Figure \ref{fig:lego+nurb}(a) and (b). To reduce the dimensionality of inputs we will use supervised pre-training to embed them in low-dimensional manifolds which will then serve as LEGOs' inputs, see Figure \ref{fig:lego+nurb}(e). We will build these manifolds via neural autoencoders and leverage contractive learning \cite{RN1070} to ensure the learned latent representations are smooth. Our preliminary studies in Figure \ref{fig:lego+nurb}(e) indicate that the supervised pre-training should achieve mean absolute errors below $10^{-8}$ to avoid information losses that propagates to LEGOs' prediction. 




